Open Vocabulary Object Detection with Proposal Mining and Prediction Equalization

Open-vocabulary object detection (OVD) aims to scale up vocabulary size to detect objects of novel categories beyond the training vocabulary. Recent work resorts to the rich knowledge in pre-trained vision-language models. However, existing methods are ineffective in proposal-level vision-language alignment. Meanwhile, the models usually suffer from confidence bias toward base categories and perform worse on novel ones. To overcome the challenges, we present MEDet, a novel and effective OVD framework with proposal mining and prediction equalization. First, we design an online proposal mining to refine the inherited vision-semantic knowledge from coarse to fine, allowing for proposal-level detection-oriented feature alignment. Second, based on causal inference theory, we introduce a class-wise backdoor adjustment to reinforce the predictions on novel categories to improve the overall OVD performance. Extensive experiments on COCO and LVIS benchmarks verify the superiority of MEDet over the competing approaches in detecting objects of novel categories, e.g., 32.6% AP50 on COCO and 22.4% mask mAP on LVIS.

==> latex/src/checklist.tex <==
\section*{Checklist}
\begin{enumerate}[leftmargin=*]
    \item For all authors...
    \begin{enumerate}
        \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
        \textcolor{blue}{[Yes]} We claim to propose a novel and effective framework for OVD task and our method achieves empirical gains over existing OVD baselines. The supportive experimental results are presented in Sec.~\ref{sec:experiments}.
        % Claims in the paper should match theoretical and experimental results in terms of how much the results can be expected to generalize.
        % The paper's contributions should be clearly stated in the abstract and introduction, along with any important assumptions and limitations. It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper.
        
        \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
        \textcolor{blue}{[Yes]}
        % Please read the ethics review guidelines.
        
        \item Did you discuss any potential negative societal impacts of your work?
        \textcolor{red}{[No]} We do not foresee any obvious negative societal impacts from our work, which contributes an open-vocabulary object detection in real-world scenario.

        \item Did you describe the limitations of your work?
        \textcolor{blue}{[Yes]} For the detailed description, please refer to Sec.~\ref{sec:ablation_investigation}.
        % You are encouraged to create a separate "Limitations" section in your paper.
    \end{enumerate}
    
    \item If you are including theoretical results...
    \begin{enumerate}
        \item Did you state the full set of assumptions of all theoretical results?
        \textcolor{red}{[No]}
        % All assumptions should be clearly stated or referenced in the statement of any theorems.
        
        \item Did you include complete proofs of all theoretical results?
        \textcolor{red}{[No]}
        % The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, authors are encouraged to provide a short proof sketch to provide intuition.
        % You are encouraged to discuss the relationship between your results and related results in the literature. 
    \end{enumerate}
    
    \item If you ran experiments...
    \begin{enumerate}
        \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
        \textcolor{blue}{[Yes]} We upload the source code in the supplementary material.
        
        \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
        \textcolor{blue}{[Yes]} We discuss all hyper-parameter tuning in Sec.~\ref{sec:ablation_investigation} and the supplementary material.
        % The full details can be provided with the code, but the important details should be in the main paper.
        
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
        \textcolor{blue}{[Yes]} The error bars are included in our main results in Sec.~\ref{sec:main_results}.
        % Answer "yes" if you report error bars, confidence intervals, or statistical significance tests for your main experiments.
        
        \item Did you include the amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
        \textcolor{blue}{[Yes]} Please refer to the details in Sec.~\ref{sec:implementation_details}.
        % Ideally, you would provide the compute required for each of the individual experimental runs as well as the total compute.
    \end{enumerate}
    
    \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
    \begin{enumerate}
        \item If your work uses existing assets, did you cite the creators?
        \textcolor{blue}{[Yes]}
        % Cite the original paper that produced the code package or dataset.
        
        \item Did you mention the license of the assets?
        \textcolor{red}{[No]}
        % State the name of the license (e.g., CC-BY 4.0) for each asset.
        
        \item Did you include any new assets either in the supplemental material or as a URL?
        \textcolor{gray}{[N/A]} Just code, which is in the supplementary material.
        % During submission time, remember to anonymize your assets. You can either create an anonymized URL or include an anonymized zip file.
        
        \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
        \textcolor{red}{[No]} We use two publicly available OVD benchmarks: COCO~\cite{coco_zeroshot} and LVIS~\cite{lvis}.
        % For example, if you collected data from via crowdsourcing, did your instructions to crowdworkers explain how the data would be used?
        % Even if you used an existing dataset, you should check how data was collected and whether consent was obtained. We acknowledge this might be difficult, so please try your best; the goal is to raise awareness of possible issues that might be ingrained in our community.
        
        \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
        \textcolor{red}{[No]} We do not use the dataset of this sort.
        % There are some settings where the existence of this information is not necessarily bad (e.g., swear words occur naturally in text). This question is just to encourage discussion of potentially undesirable properties.
    \end{enumerate}
    
    \item If you used crowdsourcing or conducted research with human subjects...
    \begin{enumerate}
        \item Did you include the full text of instructions given to participants and screenshots, if applicable?
        \textcolor{gray}{[N/A]}
        % Including this information in the supplemental material is fine, but if the main contribution of your paper involves human subjects, then we strongly encourage you to include as much detail as possible in the main paper.
        
        \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
        \textcolor{gray}{[N/A]}
        % Examples of risks include a crowdsourcing experiment which might show offensive content or collect personal identifying information (PII). Ideally, the participants should be warned.
        
        \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
        \textcolor{gray}{[N/A]}
        % First, provide the amount paid for each task (including any bonuses), and discuss how you determined the amount of time a task would take.
        % Also include discussion on how the wage was determined and how you determined that this was a fair wage.
    \end{enumerate}
\end{enumerate}

==> latex/table/tab_coco_other_15.tex <==
\begin{table}[t]
    \centering
    \vspace{-4mm}
    \setlength{\tabcolsep}{1.0mm}{
    \footnotesize{
    \begin{tabular}{l|ccc}
        \toprule
        Method & Retain & Novel & \color{gray}{All} \\
        %  & (15) & (17) & (80) \\
        \midrule
        OVR-CNN~\cite{ovrcnn}  & 11.5  & 22.9  & \color{gray}{38.1}  \\
        Detic-80~\cite{detic} & 11.5 & 27.3  & \color{gray}{38.3}  \\
        Detic-65~\cite{detic}  & 5.2 & 9.2  & \color{gray}{34.1} \\
        \midrule
        \rowcolor{gray!25} MEDet (Ours) & \textbf{18.6} & \textbf{32.6} & \color{gray}{42.4} \\
        \bottomrule
    \end{tabular}
    }
    }
    \vspace{-1mm}
    \caption{
    \textbf{Generalization on novel class.}
    %Results of COCO Novel categories.
    }
    \label{tab:coco_other_15}
    \vspace{-6mm}
\end{table}

==> latex/table/tab_effect_of_gamma_in_CBA.tex <==
\begin{table}[h]
    \centering
    \setlength{\tabcolsep}{0.8mm}{
    \footnotesize{
    \begin{tabular}{l|cccccc}
        \toprule
         & 0.0 & 0.2 & 0.4 & 0.6 & 0.8 & 1.0 \\
        \midrule
        Base  & 53.1 & 53.3 & 53.4 & 53.5 & 53.4 & 53.3 \\
        Novel & 32.0 & 32.5 & 32.6 & 32.6 & 32.6 & 32.4 \\
        \bottomrule
    \end{tabular}
    }
    }
    \caption{\textbf{The results of various $\gamma$ in CBA.}}
    \label{tab:effect_of_gamma_in_CBA}
    \vspace{-4mm}
\end{table}

==> latex/table/tab_on_COCO.tex <==
\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{1.8mm}{
    \resizebox{.98\linewidth}{!}{
    \begin{tabular}{l|cc|ccc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Detector Training}  & \multicolumn{3}{c}{COCO Generalized (48+17)} \\
        &Backbone &RPN pretrained & Novel& \color{gray}{Base} & \color{gray}{All} \\
        \midrule
        Base-only (CLIP) & - & -  & 1.3 & \color{gray}{48.7} & \color{gray}{39.3} \\
        WSDDN~\cite{wsddn} & - & - & 20.5 &\color{gray}{23.4} & \color{gray}{24.6} \\
        Cap2Det~\cite{ye2019Cap2Det} & - & -  & 20.3 & \color{gray}{20.1}  & \color{gray}{20.1} \\
        PL~\cite{rahman2020PL} & RN50-FPN & COCO Base (48) & 4.12 & \color{gray}{35.9}  & \color{gray}{27.9} \\
        OVR-CNN~\cite{ovrcnn} & RN50-C4 & COCO Base (48) & 22.8 & \color{gray}{46.0}  & \color{gray}{39.9} \\
        HierKD~\cite{hierKD} & RN50-C4 & COCO Base (48) & 20.3 & \color{gray}{51.3}  & \color{gray}{43.2} \\
        ViLD~\cite{vild} & RN50-FPN & COCO Base (48) & 27.6  & \color{gray}{59.5} & \color{gray}{51.3}\\
        RegionCLIP~\cite{regionCLIP} &RN50-C4 & LVIS (1203) & 26.8 &  \color{gray}{54.8}  & \color{gray}{47.5}\\
        Detic~\cite{detic} (reproduced) & RN50-C4 & COCO Base (48)  &28.7 \footnotesize{$\pm 0.4$} | 29.1 &  \color{gray}{52.0 \footnotesize{$\pm 0.4$} | 52.4}  &\color{gray}{45.9 \footnotesize{$\pm 0.3$} | 46.2}\\
        \midrule
        \rowcolor{gray!25} MEDet (Ours) &RN50-C4 & COCO Base (48) & \textbf{32.2 \footnotesize{$\pm 0.4$} | 32.6} &  \color{gray}{53.3 \footnotesize{$\pm 0.2$} | 53.5}  &\color{gray}{47.8 \footnotesize{$\pm 0.2$} | 48.0}\\
        \bottomrule
    \end{tabular}
    }
    \vspace{-2mm}
    \caption{\textbf{Results (mean $\pm$ variation | best) of OVD on COCO dataset~\cite{coco_zeroshot}.}
    % With a relatively simpler backbone and pre-trained RPN, 
    MEDet outperforms the others on the Novel categories.
    % The results of Detic is reproduced based on the official implementation.
    The results of MEDet are the average of five experiments.}
    \label{tab:on_COCO}
    \vspace{-4mm}
    }
\end{table}

% \begin{table}
%     \centering
%     \setlength{\tabcolsep}{1.0mm}{
%     \small{
%     \begin{tabular}{l|cc|ccc|cc}
%         \toprule
%         \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Detector Training}  & \multicolumn{3}{c|}{COCO Generalized (48+17)} & \multicolumn{2}{c}{LVIS}\\
%         &Backbone &RPN pretrained & Novel& \color{gray}{Base} & \color{gray}{All} & Novel & \color{gray}{All}\\
%         \midrule
%         Base-only (CLIP) & - & -  & 1.3 & \color{gray}{48.7} & \color{gray}{39.3} &  &  \\
%         WSDDN~\cite{wsddn} & - & - & 20.5 &\color{gray}{23.4} & \color{gray}{24.6} &16.5  &\color{gray}{30.0}  \\
%         Cap2Det~\cite{ye2019Cap2Det} & - & -  & 20.3 & \color{gray}{20.1}  & \color{gray}{20.1} &-  &-  \\
%         PL~\cite{rahman2020PL} & RN50-FPN & COCO Base (48) & 4.12 & \color{gray}{35.9}  & \color{gray}{27.9} &-  &-  \\
%         OVR-CNN~\cite{ovrcnn} & RN50-C4 & COCO Base (48) & 22.8 & \color{gray}{46.0}  & \color{gray}{39.9} &-  &-  \\
%         ViLD~\cite{vild} & RN50-FPN & COCO Base (48) &27.6  & \color{gray}{59.5} & \color{gray}{51.3} &16.6  &\color{gray}{25.6}  \\
%         RegionCLIP~\cite{regionCLIP} &RN50-C4 & LVIS (1203) & 26.8 &  \color{gray}{54.8}  & \color{gray}{47.5} &17.1  &\color{gray}{28.2}  \\
%         Detic~\cite{detic} (reproduced) & RN50-C4 & COCO Base (48)  &27.6 &  \color{gray}{50.7}  &\color{gray}{44.7} &21.3  &\color{gray}{31.0}  \\
%         \midrule
%         \rowcolor{gray!25} MEDet (Ours) &RN50-C4 & COCO Base (48) & \textbf{32.3} $\pm 0.4$ &  \color{gray}{$53.3 \pm 0.2$}  &\color{gray}{$47.8 \pm 0.2$} &  &  \\
%         \bottomrule
%     \end{tabular}
%     \vspace{-2mm}
%     \caption{\textbf{Results of OVD on the COCO~\cite{coco_zeroshot} and LVIS~\cite{lvis} dataset.} With a relatively simpler backbone and pretrained RPN, MEDet outperform the others on the Novel categories.
%     % The results of Detic is reproduced.
%     The results of MEDet are the average of five experiments.}
%     \label{tab:on_COCO}
%     \vspace{-4mm}
%     }
%     }
% \end{table}

==> latex/table/tab_on_LVIS.tex <==
\begin{table}[t]
   \centering
    \small{
    \begin{tabular}{l|cc}
        \toprule
        % \multirow{2}{*}{Method} & \multicolumn{2}{c}{LVIS} \\
        % & Novel & \color{gray}{All} \\
        Method & Novel & \color{gray}{All} \\
        \midrule
        WSDDN~\cite{wsddn} &16.5  &\color{gray}{30.0}  \\
        ViLD~\cite{vild}   &16.8  &\color{gray}{25.2}  \\
        RegionCLIP~\cite{regionCLIP} &17.1  &\color{gray}{28.2}  \\
        DetPro~\cite{DetPro} &19.8 &\color{gray}{25.9} \\
        Detic~\cite{detic} (reproduced) &21.0  &\color{gray}{30.9}  \\
        \midrule
        % \rowcolor{gray!25} MEDet (w/o CBA)  &21.3  &\color{gray}{31.0}  \\
         \rowcolor{gray!25} MEDet (Ours)  &\textbf{22.4}  &\color{gray}{34.4} \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Results on LVIS~\cite{lvis} dataset.}}
    \label{tab:on_LVIS}
    }
\end{table}

==> latex/table/tab_on_OPM.tex <==
\begin{table}[ht]
    \centering
    \footnotesize
    \begin{subtable}[t]{.8\linewidth}
        \centering
        % \resizebox{.8\linewidth}{!}{
        \setlength{\tabcolsep}{2.1mm}{
        \begin{tabular}{l|c|c|c}
            \toprule
            Method & Novel & Base & All \\
            \midrule
            Pre-trained model &17.6 &43.3 &36.6 \\
            % \midrule
            % MEDet w/o CA &29.4 &53.1 &46.9 \\ % CA: concept Augmentation
            % MEDet w/o OPM & & & \\ 
            % MEDet w/o CBA &32.0 &53.1 &47.6 \\
            % \midrule
            % MEDet w/o $\mathrm{L}_{cap}$ & & & \\
            + OPM (w/o CAug) &31.0 &52.9 &47.2\\
            + OPM  & 32.0 &53.1 &47.5  \\
            + OPM + CBA (MEDet)  &32.6 &53.4 &47.9  \\
            \midrule
            MEDet w/o $\mathrm{L}_{ramcl}$ &30.8 &52.8 &47.0 \\
            MEDet &32.6 &53.4 &47.9 \\
            \bottomrule
        \end{tabular}
        }
        \caption{}
        \label{tab:ablation_on_MEDet}
    \end{subtable}
    
    \begin{subtable}[t]{.8\linewidth}
        \centering
        % \resizebox{.8\linewidth}{!}{
        \setlength{\tabcolsep}{2.4mm}{
        \begin{tabular}{l|c|c|c}
            \toprule
            Strategy & Novel & Base & All \\
            \midrule
            % CLIP using GT &58.6 &58.2 &58.3 \\
            Top-1 $Sim$ &27.8 & 52.3 & 46.1 \\ % 直接选相似度最高的top-1
            Top-1 $SC$ &28.7 &52.6 &46.3\\ 
            Top-100 Obj &29.3 &52.4 &46.5 \\ % 直接选rpn得分的图片top-20
            \midrule
            OPM w/o $\theta_{se}$ &30.2 &53.2 &47.2 \\
            % OPM w/o TOP-3 & & & \\ % 只选择top-1
            OPM w/o merge &30.4 &52.8 &47.0 \\
            \midrule
            OPM  &31.0 &52.9 &47.2\\
            \bottomrule
        \end{tabular}
        }
        \caption{}
        \label{tab:ablation_on_OPM}
    \end{subtable}
    \caption{\textbf{(a)} \textbf{Ablation studies of MEDet.} The Line2--4 show the increase in accuracy after the addition of our proposed OPM, CAug, and CBA modules. For `MEDet w/o $\mathrm{L}_{ramcl}$' we use a cross-modal attention used in OVR~\cite{ovrcnn} to learn the vision-language knowledge.
    \textbf{(b)} \textbf{Comparison of different strategies in OPM.}}
\end{table}
